On the Four-Dimensional Formulation of Dimensionally Regulated Amplitudes

We propose a pure four-dimensional formulation (FDF) of the d-dimensional regularization of one-loop scattering amplitudes. In our formulation particles propagating inside the loop are represented by massive internal states regulating the divergences. The latter obey Feynman rules containing multiplicative selection rules which automatically account for the effects of the extra-dimensional regulating terms of the amplitude. The equivalence between the FDF and the Four Dimensional Helicity scheme is discussed. We present explicit representations of the polarization and helicity states of the four-dimensional particles propagating in the loop. They allow for a complete, four-dimensional, unitarity-based construction of d-dimensional amplitudes. Generalized unitarity within the FDF does not require any higher-dimensional extension of the Clifford and the spinor algebra. Finally we show how the FDF allows for the recursive construction of $d$-dimensional one-loop integrands, generalizing the four-dimensional open-loop approach.

==> DiagramCut/CR134.4.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Straight}{1}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Cycles}{0}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%
% Polarizzazioni
\FALabel(10.5667, 6.4667)[]{\tiny $-$}
\FALabel(8.23333, 7.6333)[]{\tiny $+$}
\FALabel(8.23333, 12.3667)[]{\tiny $-$}
\FALabel(10.5667, 13.5333)[]{\tiny $+$}
\FALabel(15., 11.1)[]{\tiny $0$}
\FALabel(15., 8.9)[]{\tiny $0$}
%
% External legs
%
\FALabel(3.1,8.)[]{\tiny$1$}
\FALabel(3.1,12.)[]{\tiny$2$}
\FALabel(17.,16.)[]{\tiny$3$}
\FALabel(17.,4.)[]{\tiny$4$}
%
\end{feynartspicture}

==> FeynmanRules/GGS_copy.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.3,8.93)[t]{\tiny $1, a, A$}
%\FALabel(5.5,8.93)[t]{\tiny $1, a, A$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b, \beta$}
\FAProp(16.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.8873,5.81315)[tr]{\tiny $3, c, \gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/P3.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,8.93)[t]{\tiny $a, A$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.2273,13.3749)[br]{\tiny $b, \beta$}
\FAProp(16.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.8873,6.01315)[tr]{\tiny $c, \gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/P4.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(3.0,13.)[]{\tiny $1,a,\alpha$}
\FAProp(4.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(3.0,7.)[]{\tiny $4,d,\delta$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(14.7868,13.4064)[]{\tiny $g_1$}
\FAProp(16.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(15.2132,8.40636)[]{\tiny $g_2$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRules/PRO.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Straight}{-1}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
\FAProp(4.,11.5)(1.5,13.0)(0.,){/GhostDash}{0}
\FAProp(4.,8.5)(1.5,7.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(18.5, 16.5)(0.,){/GhostDash}{0}
\FAProp(16.,5.)(18.5, 3.5)(0.,){/GhostDash}{0}
%
%
\end{feynartspicture}

==> FeynmanRulesCO/P3.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,8.93)[t]{\tiny $a, A$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.2273,13.3749)[br]{\tiny $b, \beta$}
\FAProp(16.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.8873,6.01315)[tr]{\tiny $c, \gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRulesCO/P4.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(3.0,13.)[]{\tiny $1,a,\alpha$}
\FAProp(4.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(3.0,7.)[]{\tiny $4,d,\delta$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(14.7868,13.4064)[]{\tiny $g_1$}
\FAProp(16.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(15.2132,8.40636)[]{\tiny $g_2$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRulesCO/PRO.1.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
\FAProp(4.,10.0)(6.5,10.0)(0.,){/Straight}{1}
\FAProp(1.,10.0)(4.,10.0)(0.,){/GhostDash}{0}
\FAProp(16.,10.0)(13.5,10.0)(0.,){/Straight}{-1}
\FAProp(16.,10.0)(19.0,10.0)(0.,){/GhostDash}{0}
%
\FAVert(6.5,10.){0}
\FAVert(13.5,10.0){0}
%
\FAProp(6.5,10.)(13.5,10.0)(0.8,){/Straight}{1}
\FAProp(6.5,10.)(13.5,10.0)(-0.8,){/Cycles}{0}
\FALabel(10.0,5.5)[]{\tiny $\bar \ell$}
%
\end{feynartspicture}

==> FeynmanRulesCO/PRO.2.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Straight}{-1}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
\FAProp(4.,11.5)(1.5,13.0)(0.,){/GhostDash}{0}
\FAProp(4.,8.5)(1.5,7.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(18.5, 16.5)(0.,){/GhostDash}{0}
\FAProp(16.,5.)(18.5, 3.5)(0.,){/GhostDash}{0}
%
%
\end{feynartspicture}

==> FeynmanRulesCO/PRO.3.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
%\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
%\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(3.5,10.0)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(1.,10.0)(3.5,10.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Cycles}{0}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Straight}{-1}
\FALabel(14.8,10.0)[]{\tiny $\bar \ell$}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%\FAProp(4.,11.5)(1.5,13.0)(0.,){/GhostDash}{0}
%\FAProp(4.,8.5)(1.5,7.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(18.5, 16.5)(0.,){/GhostDash}{0}
\FAProp(16.,5.)(18.5, 3.5)(0.,){/GhostDash}{0}
%
%
\end{feynartspicture}

==> FeynmanRulesCO/PRO.4.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
%
% External lines
%\FAProp(4.,11.5)(6.5,10.0)(0.,){/Cycles}{0}
%\FAProp(6.5,10.0)(4.,8.5)(0.,){/Cycles}{0}
\FAProp(3.5,10.0)(6.5,10.0)(0.,){/Cycles}{0}
\FAProp(1.,10.0)(3.5,10.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(13.5,13.5)(0.,){/Straight}{1}
\FAProp(16.,5.)(13.5,6.5)(0.,){/Straight}{-1}
%
% Internal lines
\FAProp(13.5,13.5)(6.5,10.0)(0.,){/Straight}{1}
\FAProp(6.5,10.0)(13.5,6.5)(0.,){/Straight}{1}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Cycles}{0}
%
% Vertices 
%
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\FAVert(6.5,10.){0}
%
%\FAProp(4.,11.5)(1.5,13.0)(0.,){/GhostDash}{0}
%\FAProp(4.,8.5)(1.5,7.0)(0.,){/GhostDash}{0}
\FAProp(16.,15.)(18.5, 16.5)(0.,){/GhostDash}{0}
\FAProp(16.,5.)(18.5, 3.5)(0.,){/GhostDash}{0}
%
\FALabel(9.5,14.0)[]{\tiny $\bar \ell +p$}
\FALabel(10.0,6.0)[]{\tiny $\bar \ell$}
%
\end{feynartspicture}

==> FeynmanRulesCO/gogo.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,10.)(16.,10.)(0.,){/GhostDash}{1}
\FALabel(5.5,8.93)[t]{\tiny $a$}
\FALabel(14.5,8.93)[t]{\tiny $b$}
\FALabel(10.,12.5)[]{\tiny $k$}
\FAVert(4.,10.){0}
\FAVert(16.,10.){0}
\end{feynartspicture}

==> FeynmanRulesCO/gogoG.tex <==
\unitlength=0.20bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(5.3,8.93)[t]{\tiny $1, a, \alpha$}
\FAProp(16.,15.)(10.,10.)(0.,){/GhostDash}{-1}
\FALabel(12.2273,13.5749)[br]{\tiny $2, b$}
\FAProp(16.,5.)(10.,10.)(0.,){/GhostDash}{1}
\FALabel(12.8873,5.81315)[tr]{\tiny $3, c$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRulesHIGGS/HGGS.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(3.0,12.)[]{\tiny $H$}
\FAProp(10.,10.)(4.,5.)(0.,){/ScalarDash}{0}
\FALabel(3.0,8.)[]{\tiny $4,D$}
\FAProp(16.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(11.,15.)[]{\tiny $2,\beta$}
\FAProp(10.,10.)(16.,5.)(0.,){/Cycles}{0}
\FALabel(11,5.)[]{\tiny $3,\gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRulesHIGGS/HSGG.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(3.0,12.)[]{\tiny $H$}
\FAProp(10.,10.)(4.,5.)(0.,){/Cycles}{0}
\FALabel(3.0,8.)[]{\tiny $4,\delta$}
\FAProp(16.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(11.,15.)[]{\tiny $2,B$}
\FAProp(10.,10.)(16.,5.)(0.,){/Cycles}{0}
\FALabel(11,5.)[]{\tiny $3,\gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRulesHIGGS/HSGS.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(3.0,12.)[]{\tiny $H$}
\FAProp(10.,10.)(4.,5.)(0.,){/ScalarDash}{0}
\FALabel(3.0,8.)[]{\tiny $4,D$}
\FAProp(16.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(11.,15.)[]{\tiny $2,B$}
\FAProp(10.,10.)(16.,5.)(0.,){/Cycles}{0}
\FALabel(11,5.)[]{\tiny $3,\gamma$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> FeynmanRulesHIGGS/HSSG.tex <==
\unitlength=0.20bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(4.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(3.0,12.)[]{\tiny $H$}
\FAProp(10.,10.)(4.,5.)(0.,){/Cycles}{0}
\FALabel(3.0,8.)[]{\tiny $4,\delta$}
\FAProp(16.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FALabel(11.,15.)[]{\tiny $2,B$}
\FAProp(10.,10.)(16.,5.)(0.,){/ScalarDash}{0}
\FALabel(11,5.)[]{\tiny $3,C$}
\FAVert(10.,10.){0}
\end{feynartspicture}

==> LeftTurning/GFF_right.tex <==
\unitlength=0.30bp%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(3.,10.)(10.,10.)(0.,){/Cycles}{0} % LEFT
\FAProp(16.,15.)(10.,10.)(0.,){/Straight}{1} % UP
\FAVert(15.8873,12.){1}
\FAProp(16.,5.)(10.,10.)(0.,){/Straight}{-1}  % DOWN
\FAVert(15.8873,8.){1}
\FAVert(10,10.){0}
\end{feynartspicture}

==> LeftTurning/GGGG.tex <==
\unitlength=0.18bp%
% X
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,10.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(10.,10.)(0.,){/Cycles}{0}
\FAVert(10.,10.){0}
%
\FAVert(18.,8.){0}
\FAVert(18.,12.){0}
\end{feynartspicture}
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(19.5,8.){0}
\FAVert(19.5,12.){0}
\end{feynartspicture}
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(10.,14.)(10.,6.)(0.,){/Cycles}{0}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(17.,7.){0}
\FAVert(17.,13.){0}
\FAVert(12.,10.){0}
\end{feynartspicture}
%
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(10.,14.)(10.,6.)(0.,){/ScalarDash}{0}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(17.,7.){0}
\FAVert(17.,13.){0}
\FAVert(12.,10.){0}
\end{feynartspicture}





==> LeftTurning/GGGG1.tex <==
\unitlength=0.18bp%
% X
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,10.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(10.,10.)(0.,){/Cycles}{0}
\FAVert(10.,10.){0}
%
\FAVert(18.,8.){0}
\FAVert(18.,12.){0}
\end{feynartspicture}
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(19.5,8.){0}
\FAVert(19.5,12.){0}
\end{feynartspicture}

==> LeftTurning/GGGG2.tex <==
\unitlength=0.18bp%
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(10.,14.)(10.,6.)(0.,){/Cycles}{0}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(17.,7.){0}
\FAVert(17.,13.){0}
\FAVert(12.,10.){0}
\end{feynartspicture}
%
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(10.,14.)(10.,6.)(0.,){/ScalarDash}{0}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(17.,7.){0}
\FAVert(17.,13.){0}
\FAVert(12.,10.){0}
\end{feynartspicture}





==> LeftTurning/GGQQ.tex <==
\unitlength=0.18bp%
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,8.){0}
\FAVert(.5,12.){0}
\end{feynartspicture}
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(3.,7.){0}
\FAVert(3.,13.){0}
\FAVert(8.,10.){0}
\end{feynartspicture}
%




==> LeftTurning/GGQQ1.tex <==
\unitlength=0.18bp%
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,8.){0}
\FAVert(19.5,8.){0}
\FAVert(10.,9.){0}
\end{feynartspicture}
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/ScalarDash}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,8.){0}
\FAVert(19.5,8.){0}
\FAVert(10.,9.){0}
\end{feynartspicture}
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(3.,7.){0}
\FAVert(17.,7.){0}
\end{feynartspicture}
%




==> LeftTurning/GGQQ2.tex <==
\unitlength=0.18bp%
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,12.){0}
\FAVert(19.5,12.){0}
\FAVert(10.,12.5){0}
\end{feynartspicture}
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/ScalarDash}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,12.){0}
\FAVert(19.5,12.){0}
\FAVert(10.,11.){0}
\end{feynartspicture}
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(3.,13.){0}
\FAVert(17.,13.){0}
\end{feynartspicture}
%




==> LeftTurning/GGQQ_right.tex <==
\unitlength=0.18bp%
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(19.5,8.){0}
\FAVert(19.5,12.){0}
\end{feynartspicture}
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(17.,7.){0}
\FAVert(17.,13.){0}
\FAVert(12.,10.){0}
\end{feynartspicture}
%




==> LeftTurning/GGQQc.tex <==
\unitlength=0.18bp%
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,8.){0}
\FAVert(19.5,8.){0}
\FAVert(10.,9.){0}
\end{feynartspicture}
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/ScalarDash}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,8.){0}
\FAVert(19.5,8.){0}
\FAVert(10.,9.){0}
\end{feynartspicture}
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(3.,7.){0}
\FAVert(17.,7.){0}
\end{feynartspicture}
%




==> LeftTurning/GGSS.tex <==
\unitlength=0.18bp%
% X
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(10.,10.)(0.,){/ScalarDash}{0}
\FAVert(10.,10.){0}
%
\FAVert(18.,8.){0}
\FAVert(18.,12.){0}
\end{feynartspicture}
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(14.,10.)(0.,){/ScalarDash}{0}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(19.5,8.){0}
\FAVert(19.5,12.){0}
\end{feynartspicture}
%
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/ScalarDash}{0}
\FAProp(10.,14.)(10.,6.)(0.,){/ScalarDash}{0}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(17.,7.){0}
\FAVert(17.,13.){0}
\FAVert(12.,10.){0}
\end{feynartspicture}





==> LeftTurning/GGSS1.tex <==
\unitlength=0.18bp%
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/ScalarDash}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/ScalarDash}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,8.){0}
\FAVert(19.5,8.){0}
\FAVert(10.,9.){0}
\end{feynartspicture}
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/ScalarDash}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,8.){0}
\FAVert(19.5,8.){0}
\FAVert(10.,9.){0}
\end{feynartspicture}
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/ScalarDash}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(3.,7.){0}
\FAVert(17.,7.){0}
\end{feynartspicture}
%




==> LeftTurning/GGSS2.tex <==
\unitlength=0.18bp%
%
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/ScalarDash}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(14.,10.)(6.,10.)(0.,){/Cycles}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,12.){0}
\FAVert(19.5,12.){0}
\FAVert(10.,11.){0}
\end{feynartspicture}
%
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/ScalarDash}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/ScalarDash}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,12.){0}
\FAVert(19.5,12.){0}
\FAVert(10.,11.){0}
\end{feynartspicture}
%
%
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/ScalarDash}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(3.,13.){0}
\FAVert(17.,13.){0}
\end{feynartspicture}
%




==> LeftTurning/GGSS3.tex <==
\unitlength=0.18bp%
% X
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,10.)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(10.,10.)(0.,){/ScalarDash}{0}
\FAVert(10.,10.){0}
%
\FAVert(18.,8.){0}
\FAVert(18.,12.){0}
\end{feynartspicture}
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(14.,10.)(0.,){/ScalarDash}{0}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(19.5,8.){0}
\FAVert(19.5,12.){0}
\end{feynartspicture}




==> LeftTurning/GGSS4.tex <==
\unitlength=0.18bp%
%
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/ScalarDash}{0}
\FAProp(10.,6.)(10.,14.)(0.,){/Cycles}{0}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(17.,7.){0}
\FAVert(17.,13.){0}
\FAVert(12.,10.){0}
\end{feynartspicture}
%
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/ScalarDash}{0}
\FAProp(10.,14.)(10.,6.)(0.,){/ScalarDash}{0}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(17.,7.){0}
\FAVert(17.,13.){0}
\FAVert(12.,10.){0}
\end{feynartspicture}





==> LeftTurning/SSQQ.tex <==
\unitlength=0.18bp%
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/ScalarDash}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/ScalarDash}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,8.){0}
\FAVert(.5,12.){0}
\end{feynartspicture}
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/ScalarDash}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/ScalarDash}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(3.,7.){0}
\FAVert(3.,13.){0}
\FAVert(8.,10.){0}
\end{feynartspicture}
%




==> RightTurning/GGQQ.tex <==
\unitlength=0.18bp%
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(19.5,8.){0}
\FAVert(19.5,12.){0}
\end{feynartspicture}
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(17.,7.){0}
\FAVert(17.,13.){0}
\FAVert(12.,10.){0}
\end{feynartspicture}
%




==> RightTurning/GQGQ.tex <==
\unitlength=0.18bp%
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Straight}{1}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/Straight}{1}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,12.){0}
\FAVert(19.5,12.){0}
\FAVert(10.,11.5){0}
\end{feynartspicture}
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(3.,13.){0}
\FAVert(17.,13.){0}
\end{feynartspicture}
%




==> RightTurning/GQSQ.n.tex <==
\unitlength=0.18bp%
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Straight}{1}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/Straight}{1}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,12.){0}
\FAVert(19.5,12.){0}
\FAVert(10.,11.5){0}
\end{feynartspicture}
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(3.,13.){0}
\FAVert(17.,13.){0}
\end{feynartspicture}
%




==> RightTurning/GQSQ.tex <==
\unitlength=0.18bp%
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Straight}{1}
\FAProp(0.,5.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(14.,10.)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{-1}
\FAProp(6.,10.)(14.,10.)(0.,){/Straight}{1}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,12.){0}
\FAVert(19.5,12.){0}
\FAVert(10.,11.5){0}
\end{feynartspicture}
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(0.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(20.,15.)(10.,14.)(0.,){/ScalarDash}{0}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(3.,13.){0}
\FAVert(17.,13.){0}
\end{feynartspicture}
%




==> RightTurning/QGQG.tex <==
\unitlength=0.18bp%
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Straight}{-1}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/Cycles}{0}
\FAProp(6.,10.)(14.,10.)(0.,){/Straight}{-1}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,8.){0}
\FAVert(19.5,8.){0}
\FAVert(10.,8.5){0}
\end{feynartspicture}
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(3.,7.){0}
\FAVert(17.,7.){0}
\end{feynartspicture}
%




==> RightTurning/QGQS.tex <==
\unitlength=0.18bp%
%
%  S
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(6.,10.)(0.,){/Straight}{-1}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{1}
\FAProp(20.,5.)(14.,10.)(0.,){/ScalarDash}{0}
\FAProp(6.,10.)(14.,10.)(0.,){/Straight}{-1}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
%
\FAVert(.5,8.){0}
\FAVert(19.5,8.){0}
\FAVert(10.,8.5){0}
\end{feynartspicture}
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Cycles}{0}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(20.,5.)(10.,6.)(0.,){/ScalarDash}{0}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(3.,7.){0}
\FAVert(17.,7.){0}
\end{feynartspicture}
%




==> RightTurning/QQQQ.tex <==
\unitlength=0.18bp%
%
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{-1}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{1}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(10.,14.)(10.,6.)(0.,){/Cycles}{0}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(3.,7.){0}
\FAVert(3.,13.){0}
\FAVert(8.,10.){0}
\end{feynartspicture}
%
% T
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{-1}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{1}
\FAProp(20.,15.)(10.,14.)(0.,){/Straight}{1}
\FAProp(20.,5.)(10.,6.)(0.,){/Straight}{-1}
\FAProp(10.,14.)(10.,6.)(0.,){/ScalarDash}{0}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
%
\FAVert(3.,7.){0}
\FAVert(3.,13.){0}
\FAVert(8.,10.){0}
\end{feynartspicture}
%



